Beauty and the beast: A case study on performance prototyping of data-intensive containerized cloud applications

Data-intensive container-based cloud applications have become popular with the increased use cases in the Internet of Things domain. Challenges arise when engineering such applications to meet quality requirements, both classical ones like performance and emerging ones like elasticity and resilience. There is a lack of reference use cases, applications, and experiences when prototyping such applications that could benefit the research community. Moreover, it is hard to generate realistic and reliable workloads that exercise the resources according to a specification. Hence, designing reference applications that would exhibit similar performance behavior in such environments is hard. In this paper, we present a work in progress towards a reference use case and application for data-intensive containerized cloud applications having an industrial motivation. Moreover, to generate reliable CPU workloads we make use of ProtoCom, a well-known library for the generation of resource demands, and report the performance under various quality requirements in a Kubernetes cluster of moderate size. Finally, we present the scalability of the current solution assuming a particular autoscaling policy. Results of the calibration show high variability of the ProtoCom library when executed in a cloud environment. We observe a moderate association between the occupancy of node and the relative variability of execution time.

==> figs/quantilessdsummaries.tex <==
> quantile(guaranteed50$V3, 0.95)
    95% 
65.8925 
> sd(guaranteed50$V3)
[1] 8.115489
> quantile(guaranteed200$V3, 0.95)
     95% 
253.0308 
> sd(guaranteed200$V3)
[1] 23.41644
> quantile(guaranteed1000$V3, 0.95)
     95% 
1166.254 
> sd(guaranteed1000$V3)
[1] 68.88045
> quantile(besteffort1000$V3, 0.95)
    95% 
1155.02 
> sd(besteffort1000$V3)
[1] 63.28705
> quantile(besteffort200$V3, 0.95)
     95% 
254.0771 
> sd(besteffort200$V3)
[1] 24.69515
> quantile(besteffort50$V3, 0.95)
    95% 
66.5653 
> sd(besteffort50$V3)
[1] 8.965577

> mean(besteffort50$V3)
[1] 52.58131
> mean(besteffort50$V3)
[1] 52.58131
> mean(guaranteed50$V3)
[1] 54.06818
> mean(besteffort200$V3)
[1] 211.0581
> mean(guaranteed200$V3)
[1] 214.5613
> mean(besteffort1000$V3)
[1] 1042.363
> mean(guaranteed1000$V3)
[1] 1042.841
> median(besteffort50$V3)
[1] 52.248
> median(guaranteed50$V3)
[1] 54.102
> median(besteffort200$V3)
[1] 206.769
> median(guaranteed200$V3)
[1] 212.349
> median(besteffort1000$V3)
[1] 1033.147
> median(guaranteed1000$V3)
[1] 1032.238





